Learning Contraction Policies from Offline Data

This paper proposes a data-driven method for learning convergent control policies from offline data using Contraction theory. Contraction theory enables constructing a policy that makes the closed-loop system trajectories inherently convergent towards a unique trajectory. At the technical level, identifying the contraction metric, which is the distance metric with respect to which a robot's trajectories exhibit contraction is often non-trivial. We propose to jointly learn the control policy and its corresponding contraction metric while enforcing contraction. To achieve this, we learn an implicit dynamics model of the robotic system from an offline data set consisting of the robot's state and input trajectories. Using this learned dynamics model, we propose a data augmentation algorithm for learning contraction policies. We randomly generate samples in the state-space and propagate them forward in time through the learned dynamics model to generate auxiliary sample trajectories. We then learn both the control policy and the contraction metric such that the distance between the trajectories from the offline data set and our generated auxiliary sample trajectories decreases over time. We evaluate the performance of our proposed framework on simulated robotic goal-reaching tasks and demonstrate that enforcing contraction results in faster convergence and greater robustness of the learned policy.

==> preliminaries.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.4\textwidth]{Fig/contraction.jpg}
    \caption{Contraction of two close trajectories.}
    \label{fig:contraction}
\end{figure}

Contraction theory introduces a domain of differentiable dynamic systems $\mathcal{F}$ that the state trajectories of a system $g \in \mathcal{F}$ separated by an infinitesimally small distance at the initial condition tend to converge as they evolve in time. Figure~\ref{fig:contraction} demonstrates a graphical notion of contraction. Formally, a discrete-time dynamic system $g(\x): \real^n \to \real^n$ defined as
\begin{align}\label{eq::mainDynamics}
    \xtpl=g(\xt), 
\end{align} 
is \emph{contracting}  if for any infinitesimal state perturbation $\dxt$ at any time $t$ the system satisfies
\begin{align}\label{eq::contractionSimp}
    \Lnorm \dxt \Rnorm^2 > \Lnorm g(\xprt) - g(\xt) \Rnorm^2,
\end{align}
where $\xprt = \xt + \dxt$. That is, the distance of two infinitesimally close states gets smaller in forward time~\cite{WL-JJES:98}.

For an infinitesimally small perturbations, first order Taylor expansion allows us to related locally the trajectories of the perturbed and unperturbed system via the system Jacobian $\nabla g(\xt) = \left.\frac{\partial g(\x)}{\partial \x} \right\vert_{\x=\xt}$, i.e., 
\begin{align}\label{eq::diffEq}
    g(\xprt) - g(\xt) = \nabla g(\xt) \dxt.
\end{align}
Using~\eqref{eq::diffEq}, the contraction condition~\eqref{eq::contractionSimp} can be restated as 
\begin{align}\label{eq::ineqSimp}
    \dxt^\top \dxt > \dxt^\top \nabla g(\xt)^\top \nabla g(\xt)\dxt.
\end{align}
The reader can confirm that a sufficient for~\eqref{eq::ineqSimp}, and thus~\eqref{eq::mainDynamics} being contracting is  
\begin{align}\label{eq::ineqSimp2}
    \nabla g(\xt)^\top \nabla g(\xt) \leq -\beta \Id,
\end{align}
for a $\beta \in \realpositive$. A more general contraction condition can be obtained by using a full rank state dependant metric $\T(\x), \,\,\, \x \in \real^n$ to write the contraction condition as 
\begin{align}\label{eq::contCond}
    \Lnorm \T(\xt)\dxt \Rnorm^2 > \Lnorm \T(\xtpl)\left(g(\xprt) - g(\xt) \right)\Rnorm^2,
\end{align}
or equivalently, 
\begin{align}\label{eq::ineqGen}
    \dxt^\top \M(\xt) \dxt > \dxt^\top\Big( \nabla g(\xt)^\top \M(\xtpl)\nabla f(\xt)\Big)\dxt.
\end{align}
where $\M(\x) = \T(\x)^\top \T(\x)$.
Thus, for dynamical system~\eqref{eq::mainDynamics} to be contracting, the sufficient condition is the existence of $\Mx > 0$ such that

\begin{align}\label{eq::ineqGen2}
\nabla g(\xt)^\top \M(\xtpl) \nabla g(\xt)-\M(\xt) < 0 
\end{align}
